Automated Prompt Generation for Code Intelligence: An Empirical study and Experience in WeChat

Large Code Models (LCMs) show potential in code intelligence, but their effectiveness is greatly influenced by prompt quality. Current prompt design is mostly manual, which is time-consuming and highly dependent on specific LCMs and tasks. While automated prompt generation (APG) exists in NLP, it is underexplored for code intelligence. This creates a gap, as automating the prompt process is essential for developers facing diverse tasks and black-box LCMs. To mitigate this, we empirically investigate two important parts of APG: Instruction Generation (IG) and Multi-Step Reasoning (MSR). IG provides a task-related description to instruct LCMs, while MSR guides them to produce logical steps before the final answer. We evaluate widely-used APG methods for each part on four open-source LCMs and three code intelligence tasks: code translation (PL-PL), code summarization (PL-NL), and API recommendation (NL-PL).Experimental results indicate that both IG and MSR dramatically enhance performance compared to basic prompts. Based on these results, we propose a novel APG approach combining the best methods of the two parts. Experiments show our approach achieves average improvements of 28.38% in CodeBLEU (code translation), 58.11% in ROUGE-L (code summarization), and 84.53% in SuccessRate@1 (API recommendation) over basic prompts. To validate its effectiveness in an industrial scenario, we evaluate our approach on WeChat-Bench, a proprietary dataset, achieving an average MRR improvement of 148.89% for API recommendation.

==> figures/CoT_Prompt.tex <==
\begin{figure}[htbp]
    \centering
    \caption{CoT prompt for code translation and code summary} \label{fig:cot_prompt}
    \begin{promptbox}{CoT Prompt Template}
        \textbf{Generate comments for \textcolor{purple}{[LANG]} code. /} 
        \textbf{Translate the \textcolor{purple}{[SOURCE\_LANG]} code to \textcolor{blue}{[TARGET\_LANG]}.} \\
        \textbf{\$ Example Code} \\
        \textbf{Let's think step by step.}\\
        1. reasoning step one. \\
        2. reasoning step two. \\
        ... \\
        N. reasoning step N.\\
        \textbf{Therefore the translation/summarization is:} \\
        \textbf{[Answer]} \\
        \textbf{\$ Input Code:} \\
        \textbf{\$ Output Answer}
    \end{promptbox}
\end{figure}
